CHSM8: A Chess Transformer that Follows Natural-Language Style Prompts

We present CHSM8, a 210M-parameter chess transformer that plays moves conditioned on a free-text description of a playing style, e.g. "go for the Sicilian Defense", "solid, safe, risk-free chess" or "You are Magnus Carlsen in his prime". The model is pretrained without search on 1.07B filtered Lichess games, using a factorized move representation and legal-move masking. It reaches 1837 Elo against a strength-limited Stockfish and, in 1,000-game matches, beat every other public model we tested that was likewise trained without preference tuning, rewards or search, including one with 13 times as many parameters. We then fine-tune it to follow text on a synthetic dataset: Gemma-4-31B describes the playing style of 3M game sides, a 1B Gemma-3 model distilled from the 2.4M of those descriptions that contradict nothing on the board labels the rest, and every one of 30M selected game sides gets five descriptions. Supervised fine-tuning attaches a frozen text encoder through gated cross-attention, and direct preference optimization (DPO) uses the same moves under a mismatched description as the rejected sample. After DPO, style adherence rises on every prompt we test (for example, queens traded early 53% -> 67%, pawn moves 29% -> 32% of all moves, queenside castling 97.3% -> 99.7%), and strength without a prompt stays within noise of SFT (1792 vs. 1797 Elo). Design choices at every stage were made by fixed-budget automated search loops on top of standard architectures and training recipes. We document the full pipeline and the decisions behind it, report the ablations that failed, and evaluate the models across many style prompts and kinds of games, with 1,000 games per setting. The work is fully open source and reproducible: weights, datasets with all training labels, prompts, configurations, inference code and playable demos are public and free to build on.

==> floats/tab-fullpass.tex <==
\begin{table}[H]
\centering\small
\input{tables/fullpass.tex}
\caption{Checkpoints along the full DPO pass (random band), 1,000 games per prompt.}
\label{tab:fullpass}
\end{table}


==> floats/tab-longband.tex <==
\begin{table}[H]
\centering\small
\input{tables/longband.tex}
\caption{Checkpoints along the long-band-only DPO pass, 1,000 games per prompt.}
\label{tab:longband}
\end{table}


==> sections/pilot.tex <==
\section{A pilot of the CLIP-reward PPO plan}\label{sec:pilot}
Before the full label corpus existed, we tested the originally planned post-training pipeline on a 100k-side pilot
(50k Gemma and 50k Apertus labels, split by game).
For this we used intermediate pretraining checkpoints.

\paragraph{SFT.}
A small text tower was trained from scratch: a word-level tokenizer and a two-layer bidirectional transformer.
It fed the decoder's cross-attention through a zero-initialized scalar gate.
The best recipe used three learning rates:
\begin{itemize}\setlength\itemsep{0pt}
\item $3{\times}10^{-6}$ for the pretrained chess body;
\item $10^{-5}$ for the never-trained cross-attention path;
\item $3{\times}10^{-5}$ for the text tower.
\end{itemize}
After 12 minutes, the right-minus-wrong cross-entropy gap was only $-0.012$.
Initializing cross-attention from the same layer's self-attention weights was clearly worse, and so was initializing the
text tower from the contrastive model below.

\paragraph{Chess-CLIP.}
A two-tower contrastive model \citep{radford2021clip,oord2018cpc} paired the text tower with the chess body.
Only the last chess block was trainable, and the chess tower pooled the hidden states at the described side's moves.
On 5,039-way validation retrieval it reached R@1 1.4--1.5\% (about 75$\times$ chance) and a median rank of about 465,
with two independently seeded models in agreement.

\paragraph{PPO.}
We ran legal whole-move PPO \citep{schulman2017ppo} with alternating self-play rollouts, a frozen SFT opponent and
reference, and a grouped advantage estimator in the style of GRPO \citep{shao2024grpo}.
The CLIP model provided the reward, and an independently seeded second CLIP served as an audit.
Across learning rates from $10^{-6}$ to $3{\times}10^{-5}$, neither the training reward nor the audit reward moved beyond
$\pm0.001$, while validation loss got worse.

The conclusion was that the reward was too weak to optimize against.
We shelved PPO in favour of improving SFT and, later, DPO on the labeled data (\cref{sec:dpo}), which needs no reward
model.


==> tables/fullpass.tex <==
\begin{tabular}{lrrrrr}
\toprule
checkpoint & queens (\%) & pawns & queenside (\%) & Elo, none & attack gap \\
\midrule
SFT & 51.3 & .292 & 97.1 & 1789 & $-41$ \\
25\% & 58.1 & .317 & 99.7 & 1811 & $-134$ \\
50\% & 61.4 & .320 & 99.7 & 1774 & $-91$ \\
75\% & 56.9 & .317 & 99.8 & 1790 & $-118$ \\
100\% & 57.1 & .319 & 99.6 & 1807 & $-159$ \\
\bottomrule
\end{tabular}


==> tables/longband.tex <==
\begin{tabular}{lrrrrr}
\toprule
checkpoint & queens (\%) & pawns & queenside (\%) & Elo, none & attack gap \\
\midrule
SFT & 51.3 & .292 & 97.1 & 1789 & $-41$ \\
25\% & 63.0 & .318 & 99.1 & 1776 & $-98$ \\
50\% & 62.8 & .312 & 99.7 & 1789 & $-96$ \\
75\% & 60.0 & .311 & 99.7 & 1799 & $-113$ \\
100\% & 61.5 & .306 & 99.4 & 1784 & $-92$ \\
\bottomrule
\end{tabular}

